Matching Dyadic Distributions to Channels

Many communication channels with discrete input have non-uniform capacity achieving probability mass functions (PMF). By parsing a stream of independent and equiprobable bits according to a full prefix-free code, a modu-lator can generate dyadic PMFs at the channel input. In this work, we show that for discrete memoryless channels and for memoryless discrete noiseless channels, searching for good dyadic input PMFs is equivalent to minimizing the Kullback-Leibler distance between a dyadic PMF and a weighted version of the capacity achieving PMF. We define a new algorithm called Geometric Huffman Coding (GHC) and prove that GHC finds the optimal dyadic PMF in O(m \log m) steps where m is the number of input symbols of the considered channel. Furthermore, we prove that by generating dyadic PMFs of blocks of consecutive input symbols, GHC achieves capacity when the block length goes to infinity.

==> Makefile <==
PROJECT=geometric
TMPFILES=*.aux *.bak *.bbl *.blg *.lof *.log *.toc *.lot *~ *.backup\
*.pfx *.ovp $(PROJECT)-pics.* $(PROJECT).dvi $(PROJECT).ps
ARXIVTMP=*.aux *.bak *.blg *.lof *.log *.toc *.lot *~ *.backup\
*.pfx *.ovp $(PROJECT)-pics.* $(PROJECT).dvi $(PROJECT).ps $(PROJECT).pdf *.bib .*.xml

default:
	latex $(PROJECT).tex;

clean:
	rm -f $(TMPFILES);

clean_pdf:
	rm -f $(PROJECT).pdf;

final: clean clean_pdf
	pdflatex $(PROJECT).tex;
	pdflatex $(PROJECT).tex;
	bibtex $(PROJECT);
	pdflatex $(PROJECT).tex;
	pdflatex $(PROJECT).tex;

literatur:
	cp ../references/Dnc.bib ./;
	cp ../references/confs-jrnls.bib ./;
	cp ../references/IEEEabrv.bib ./;
	cp ../references/IEEEtran.cls ./;
	cp ../references/IEEEtran.bst ./;

arxiv:
	rm -f $(ARXIVTMP);
	rm -rf .git;


==> problem.tex <==
\section{Problem Statement}

Consider a binary sequence $(B_k,k\in\mathbb{N})$ where the $B_k$ are IID according to $\probop(B_k=0)=\probop(B_k=1)=\frac{1}{2}$. This binary stream can be parsed by a dictionary obtained from a full binary tree. The binary tree is specified by the wordlengths $\pmb{\ell}$. The words in the dictionary are generated according to the induced PMF $\pmb{p}$, where $p_i=2^{-\ell_i}$ for all $i$. We define the set $\mathbb{D}$ of dyadic PMFs as
\begin{align}
\mathbb{D}=\{\vecp\,|\,\vecp&\text{ is a PMF},\nonumber\\
&\text{for } i=1,\dotsc,m:p-i=2^{-\ell_i},\ell_i\in\mathbb{N}\}
\end{align}
We now interested in dyadic PMFs $\vecp\in\mathbb{D}$ that approximate capacity achieving distributions well with respect to an appropriate information-theoretic distance measure.


==> stairway.tex <==
\section{Boundedness of \textsc{Gcc}}
\label{sec:swc}

We will now define an algorithm that guarantees $\kl(\vecp\Vert\vecp^*)\leq 1$.
The idea is to assign $\ell_i=\lfloor -\log p_i^*\rfloor$. However, since $\sum_{i=1}^n p_i^*=1$, $\sum_{i=1}^n 2^{-\lfloor -\log p_i^*\rfloor}$ may exceed one and violate Kraft's inequality \cite[Theorem 2.3.1]{Gallager2008}. In this case, there is no prefix-free code with word lengths $\lfloor -\log p_i^*\rfloor$. We circumvent this problem in the following way. First, we sort $\vecp^*$ such that $p^*_1\geq p^*_2 \geq\dotsb\geq p^*_n$. We then assign $\ell_i=\lfloor -\log p_i^*\rfloor$ for $i\leq k$ and $\ell_i=\infty$ for $i>k$, where $k\leq n$ is chosen such that
\begin{align}
\sum\limits_{i=1}^k 2^{-\ell_i}=1.
\end{align}
This scheme is stated in Algorithm~\ref{alg:swc}. The following lemma shows that Algorithm~\ref{alg:swc} is well-defined.
%
%
%
%
%
\begin{lemma}
Algorithm~\ref{alg:swc} constructs a full prefix-free code.
\end{lemma}
\begin{proof}
Define $\pmb{\ell}^{(k)}=(\ell_1,\dotsc,\ell_k)$ and $L_k=\sum_{i=1}^k2^{-\ell_i}$. By \cite[Theorem 2.3.1]{Gallager2008}, $\pmb{\ell}^{(k)}$ is a full prefix-free code if and only if $L_k=1$. We thus have to show that $L_k=1$ for some $k\leq n$. First, it holds that
\begin{align}
\sum\limits_{i=1}^n 2^{-\ell_i} \geq \sum\limits_{i=1}^n 2^{-w_i} = \sum\limits_{i=1}^n q =1
\end{align}
thus, there exists a $k\leq n$ such that $L_k\geq 1$. It remains to show that $L_k$ is exactly equal to $1$ for some $k\leq n$. This follows from the claim that for any $k$ with $L_k< 1$, $1-L_k$ is a nonnegative multiple of $2^{-\ell_{k+1}}$. Thus, $1-L_{k+1}=(1-L_k)-2^{-\ell_{k+1}}\geq 0$, i.e., 
\begin{align}
L_k<1\Rightarrow L_{k+1}\leq 1. 
\end{align}
Since $\ell_{k+1}=\ell_k+t$ for some integer $t\geq 0$, $1-L_k$ is a multiple of $2^{-\ell_{k+1}}$ if it is a multiple of $2^{-\ell_k}=2^{-\ell_{k+1}}2^t$. We show the latter by induction in $k$.\\
\emph{}
\emph{Induction basis:} For $k=1$, $1-L_1=1-2^{-\ell_1}=(2^{\ell_1}-1)2^{-\ell_1}$.\\
\emph{Induction step:} Assume $1-L_k=s\cdot 2^{-\ell_k}$ for some integer $s>0$. For some integer $t\geq 0$, it holds that $\ell_{k+1}=\ell_k+t$. Now 
\begin{align}
1-L_{k+1}=1-L_k-2^{-\ell_{k+1}}=s\cdot 2^{-\ell_k}-2^{-\ell_{k+1}}&=s\cdot 2^{-(\ell_{k+1}-t)}-2^{-\ell_{k+1}}\nonumber\\
&=(s2^{t}-1) 2^{-\ell_{k+1}}
\end{align}
\end{proof}
%
%
%
\begin{proposition}\label{prop:ao}
Denote by $\vecp^*$ an arbitrary PMF with $n$ entries. For input $\vecp^*$, denote by $\vecp$ the output of Algorithm~\ref{alg:swc}. Then $\kl(\vecp\Vert\vecp^*)\leq 1$.
\end{proposition}
\begin{proof}
\begin{align}
\kl(\pmb{p}\Vert\vecp^*)=\sum\limits_{i=1}^{n} p_i\log\frac{p_i}{p_i^*}
&\leq\sum\limits_{i=1}^{n} p_i\log\frac{2^{-\lfloor -\log p^*_i\rfloor}}{p_i^*}\\
&\leq\sum\limits_{i=1}^{n} p_i\log\frac{2^{-( -\log p^*_i-1)}}{p_i^*}\\
&=\sum\limits_{i=1}^{n} p_i \log\frac{2p_i^*}{p^*_i}\\
&=1.
\end{align}
\end{proof}
\begin{remark}
Huffman source codes achieve for $m\rightarrow\infty$ the maximum compression rate of $1$ information bit per codeword bit. This can be shown by using the Shannon code $\ell_i=\lceil-\log p^*_i\rceil$, defining the induced PMF as $p_i=2^{-\ell_i}/\sum_i 2^{-\ell_i}$ and showing that $\kl(\vecp^*\Vert\vecp)\leq 1$.
\end{remark}

